Modular implicits

We present modular implicits, an extension to the OCaml language for ad-hoc polymorphism inspired by Scala implicits and modular type classes. Modular implicits are based on type-directed implicit module parameters, and elaborate straightforwardly into OCaml's first-class functors. Basing the design on OCaml's modules leads to a system that naturally supports many features from other languages with systematic ad-hoc overloading, including inheritance, instance constraints, constructor classes and associated types.

==> eptcsdata.tex <==
\providecommand{\firstpage}{22}
\providecommand{\publicationstatus}{Kiselyov and Garrigue (Eds.): ML Family/OCaml Workshops 2014.\\
EPTCS 198, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.198.2}{10.4204/EPTCS.198.2}}

